A Reduced Basis Technique for Long-Time Unsteady Turbulent Flows

We present a reduced basis technique for long-time integration of parametrized incompressible turbulent flows. The new contributions are threefold. First, we propose a constrained Galerkin formulation that corrects the standard Galerkin statement by incorporating prior information about the long-time attractor. For explicit and semi-implicit time discretizations, our statement reads as a constrained quadratic programming problem where the objective function is the Euclidean norm of the error in the reduced Galerkin (algebraic) formulation, while the constraints correspond to bounds for the maximum and minimum value of the coefficients of the $N$-term expansion. Second, we propose an \emph{a posteriori} error indicator, which corresponds to the dual norm of the residual associated with the time-averaged momentum equation. We demonstrate that the error indicator is highly-correlated with the error in mean flow prediction, and can be efficiently computed through an offline/online strategy. Third, we propose a Greedy algorithm for the construction of an approximation space/procedure valid over a range of parameters; the Greedy is informed by the \emph{a posteriori} error indicator developed in this paper. We illustrate our approach and we demonstrate its effectiveness by studying the dependence of a two-dimensional turbulent lid-driven cavity flow on the Reynolds number.

==> bib_folder/old_bib.tex <==
@book{adams2003sobolev,
  title={Sobolev spaces},
  author={Adams, R A and Fournier, J  JF},
  volume={140},
  year={2003},
  publisher={Academic press}
}

@book{pinkus1985n,
  title={N-widths in Approximation Theory},
  author={Pinkus, A},
  volume={7},
  year={1985},
  publisher={Springer Science \& Business Media}
}


@Book{wiener_filtering,
author = {J. S.  Lim},
publisher = {Prentice Hall},
title = {Two-dimensional signal and image processing},
year = {1990},
}

@article{maday2015pbdw,
  title={PBDW State Estimation: Noisy Observations; Configuration-Adaptive Background Spaces; Physical Interpretations},
  author={Maday, Y and Patera, A  T and Penn, J D and Yano, M},
  journal={ESAIM: Proceedings and Surveys},
  volume={50},
  pages={144--168},
  year={2015},
  publisher={EDP Sciences}
}

@book{hewitt2012abstract,
  title={Abstract Harmonic Analysis: Volume I Structure of Topological Groups Integration Theory Group Representations},
  author={Hewitt, E and Ross, K A},
  volume={115},
  year={2012},
  publisher={Springer Science \& Business Media}
}

@book{hastie2009elements,
  title={The elements of statistical learning},
  author={Hastie, T. and Tibshirani, R. and Friedman, J.},
  volume={2},
  number={1},
  year={2009},
  publisher={Springer}
}

@book{rice2006mathematical,
  title={Mathematical statistics and data analysis},
  author={Rice, J},
  year={2006},
  publisher={Cengage Learning}
}

@book{jacod2003probability,
  title={Probability essentials},
  author={Jacod, J. and Protter, P. E},
  year={2003},
  publisher={Springer}
}
@article{babuska2011optimal,
  title={Optimal local approximation spaces for generalized finite element methods with application to multiscale problems},
  author={Babuska, I  and Lipton, R },
  journal={Multiscale Modeling \& Simulation},
  volume={9},
  number={1},
  pages={373--406},
  year={2011},
  publisher={SIAM}
}

==> sezioni/dual_norm_idea.tex <==
The goal here is to reduce the cost associated with the computation of the residual.
I recall that our main concern is related to offline storage. I will consider here a simplified task, which I still believe is of some interest.


\textbf{Task:} given the functional $\ell(v; \mu)= \sum_{m=1}^M \, \Theta_m(\mu) \ell_q(v)$, we want to estimate
$\|   \ell(\cdot, \mu) \|_{\star} = {\rm arg} \max_{v \in \mathcal{X}} \frac{\ell(v; \mu)}{\|  v \|}$. We consider the case in which 
$\Theta_m(\mu)$ can be evaluated rapidly.

\textbf{Option 1(standard approach):}
observe that $\ell(v; \mu) = \sum_{m=1}^M \Theta_m(\mu) (\xi_q,   v)$ where 
$\xi_q$ is the Riesz representer associated with $\ell_q$.
The offline cost scales with $\mathcal{O}( M \mathcal{N}^d   )$ where $d>1$ corresponds to the solution to a sparse linear system.
The storage cost is $\mathcal{O}(M \mathcal{N})$, which might be huge.


\textbf{Option 2 (my tentative proposal):}
Estimate $\|   \ell(\cdot, \mu) \|_{\star}  \approx {\rm arg} \max_{v \in  X} \frac{\ell(v; \mu)}{\|  v \|}$, where 
${\rm dim}(X) = K \ll \mathcal{N}$.
The offline cost scales with $\mathcal{O}( M K^3   )$.
The storage cost is $\mathcal{O}(M K)$ (to store the reduced Riesz representers) + $\mathcal{O}(K \mathcal{N})$ (to store $X$).
If $K < M$ then the approach is convenient. 


\textbf{Question:} how to choose $X$? One natural choice is to sample $\mu^1,\ldots, \mu^K \in \mathcal{P}$, compute
the Riesz representers $\tilde{\xi}^1,\ldots, \tilde{\xi}^K$, and then define 
$X={\rm span}\{ \tilde{\xi}^1,\ldots, \tilde{\xi}^K \}$.

\begin{enumerate}
\item
Can we say something about the error a priori?
This is completely standard.
Let $\mu \in \mathcal{P}$, and let $\xi(\mu) \in \mathcal{X}$ be the Riesz representer associated with $\ell(\cdot; \mu)$.
Then, we find
$$
\| \ell(\cdot; \mu) \|_{X'} = \|  \Pi_X \xi(\mu)    \|.
$$
Therefore,
$$
\|   \ell(\cdot, \mu) \|_{\star}^2
-
\|   \ell(\cdot, \mu) \|_{X'}^2
=
\|  \Pi_{X^{\perp}}  \xi(\mu)  \|^2.
$$
\item
Can we say something about the error a posteriori?
We can use standard cross-validation or holdout validation procedures to assess performance. These approaches will provide us with estimates of $\| 
\|   \ell(\cdot, \mu) \|_{\star} 
-
\|   \ell(\cdot, \mu) \|_{X'} 
\|_{L^2(\mathcal{P})}$.
\item
Straightforward implementations require the storage of $\mathcal{O}(K \mathcal{N})$.
However, we might perform a (live-approximate) HAPOD   to reduce the dimension of $X$ in run-time.
This might reduce quite dramatically the offline storage.
\item
For nonlinear unsteady problems, the computation of $\Theta_m$ is not   inexpensive.
The key assumption here is that we can compute reasonably good reduced spaces $X$ even based on approximate values for 
$\Theta_m(\mu)$ (i.e., shorter time integration, low-dimensional approximations). As usual, this reduces to the assessment of the robustness of our approach to perturbation...
\item
It seems to me that in the pMOR community this problem has not been addressed (am I right about that?).
On the other hand, 
the idea proposed here has already  been explored in the  dynamic programming community/Monte Carlo linear algebra community.
In this respect,I found a presentation by Bertsekas \url{www.mit.edu/~dimitrib/Monte_Carlo_Linear_Algebra.pdf} that addresses a similar problem and uses a similar idea (basically he resorts to projection onto a reduced space, which is essentially the same as I propose). 
A representative (and quite recent) paper about this topic is
\cite{bertsekas2009projected}.
\end{enumerate}




